SpaceJAM: a Lightweight and Regularization-free Method for Fast Joint Alignment of Images

The unsupervised task of Joint Alignment (JA) of images is beset by challenges such as high complexity, geometric distortions, and convergence to poor local or even global optima. Although Vision Transformers (ViT) have recently provided valuable features for JA, they fall short of fully addressing these issues. Consequently, researchers frequently depend on expensive models and numerous regularization terms, resulting in long training times and challenging hyperparameter tuning. We introduce the Spatial Joint Alignment Model (SpaceJAM), a novel approach that addresses the JA task with efficiency and simplicity. SpaceJAM leverages a compact architecture with only 16K trainable parameters and uniquely operates without the need for regularization or atlas maintenance. Evaluations on SPair-71K and CUB datasets demonstrate that SpaceJAM matches the alignment capabilities of existing methods while significantly reducing computational demands and achieving at least a 10x speedup. SpaceJAM sets a new standard for rapid and effective image alignment, making the process more accessible and efficient. Our code is available at: https://bgu-cs-vil.github.io/SpaceJAM/.

==> figures/main_fig.tex <==

\begin{tikzpicture}[node distance=1cm and 0.5cm, auto]

  % Define styles
  \tikzset{
    image/.style={rectangle, draw, fill=white, inner sep=0pt, minimum size=1.25cm},
    process/.style={rectangle, draw, fill=blue!20, text width=1.5cm, text centered, minimum height=1.25cm},
    arrow/.style={-Latex}
  }

  % Column 1 - Input Images
  \node[image] (img1) {\includegraphics[width=.05\textwidth]{placeholder1}};
  \node[image, below=of img1] (img2) {\includegraphics[width=.05\textwidth]{placeholder2}};
  \node[image, below=of img2] (img3) {\includegraphics[width=.05\textwidth]{placeholder3}};
  \node[image, below=of img3] (img4) {\includegraphics[width=.05\textwidth]{placeholder4}};
  
  % Column 2 - DINO ViT
  \node[process, right=of img2, yshift=0.5cm] (dino1) {DINO ViT};
  \node[process, right=of img3, yshift=-0.5cm] (dino2) {DINO ViT};

  % Column 3 - DINO keys and Saliency masks
  \node[image, right=of dino1, xshift=0.5cm] (key1) {\includegraphics[width=.05\textwidth]{placeholder5}};
  \node[image, right=of key1] (mask1) {\includegraphics[width=.05\textwidth]{placeholder6}};
  \node[image, right=of dino2, xshift=0.5cm] (key2) {\includegraphics[width=.05\textwidth]{placeholder7}};
  \node[image, right=of key2] (mask2) {\includegraphics[width=.05\textwidth]{placeholder8}};

  % Column 4 - STN
  \node[process, right=of mask1, xshift=1cm] (stn) {STN};

  % Column 5 - Congealed images and features
  \node[image, right=of stn, xshift=1cm] (congealed1) {\includegraphics[width=.05\textwidth]{placeholder9}};
  \node[image, below=of congealed1] (congealed2) {\includegraphics[width=.05\textwidth]{placeholder10}};

  % Column 6 - Joint Atlas
  \node[process, right=of congealed1, xshift=1cm] (atlas) {Joint Atlas};
  
  % Arrows
  \draw[arrow] (img1) -- (dino1);
  \draw[arrow] (img2) -- (dino1);
  \draw[arrow] (img3) -- (dino2);
  \draw[arrow] (img4) -- (dino2);
  \draw[arrow] (dino1) -- (key1);
  \draw[arrow] (dino1) -- (mask1);
  \draw[arrow] (dino2) -- (key2);
  \draw[arrow] (dino2) -- (mask2);
  \draw[arrow] (mask1) -- (stn);
  \draw[arrow] (mask2) -- (stn);
  \draw[arrow] (stn) -- (congealed1);
  \draw[arrow] (stn) -- (congealed2);
  \draw[arrow] (congealed1) -- (atlas);

  % Labels
  \node[above=0.5cm of img1] {(a) Input};
  \node[above=0.5cm of key1] {(b) DINO-ViT features};
  \node[above=0.5cm of congealed1] {(c) Congealed images and features};
  \node[above=0.5cm of atlas] {(d) Joint Atlas};

\end{tikzpicture}


==> macros.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would 
% not end up as ``with respect toblah''. 
 
\def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
\def\etal{\emph{et al}\onedot}
% \def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------

\newcommand{\FIG}{Fig.~}
\newcommand{\FIGS}{Figs.~}
\newcommand{\EQN}{Eq.~}
% \newcommand{\EQN}{Equation }
\newcommand{\EQNS}{Eqs.~}
% \newcommand{\EQNS}{Equations }

%\newcommand{\SEC}{Sec.~}.  Use \autoref or ~\autoref instead.



% integers
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\Rtwo}{\ensuremath{\RR^2}}
\newcommand{\Rthree}{\ensuremath{\RR^3}}
\newcommand{\Rfive}{\ensuremath{\RR^5}}

\newcommand{\Rsix}{\ensuremath{\RR^6}}

\newcommand{\Rn}{\ensuremath{\RR^n}}
\newcommand{\Rd}{\ensuremath{\RR^d}}
\newcommand{\Rk}{\ensuremath{\RR^k}}

% 
%positive integers
\newcommand{\Zplus}{\ensuremath{\ZZ^+}}
%positive reals
\newcommand{\Rplus}{\ensuremath{\RR^+}}


% set notation
% \newcommand{\set}[1]{\ensuremath{{\left\{#1\right\}}}}
\newcommand{\set}[1]{\ensuremath{{\{#1\}}}}
\newcommand{\tuple}[1]{\ensuremath{{(#1)}}}
\newcommand{\tupleLarge}[1]{\ensuremath{{\left(#1\right)}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}



\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\sign}[1]{{\mathrm{sign}\left(#1\right)}}

\newcommand{\ellTwo}{\ell_2}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellOne}{\ell_1}




\newcommand{\MATRIX}[2][cccccccccccccccccccc]{\left[
 \begin{array}{#1}
 #2
 \end{array}
\right]}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}



% homogeneous coordinates
\newcommand{\bxh}{\widetilde{\bx}}

\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}
\newcommand{\GREEN}[1]{{{\color{green}{#1}}}}
\newcommand{\MAGENTA}[1]{{{\color{magenta}{#1}}}}  



\newcommand{\FREIFELD}[1]{\textbf{\MAGENTA{[FREIFELD says: #1]}}}
% Make your own

\newcommand{\TBD}{\RED{[TBD]}}
\newcommand{\TODO}[1]{\RED{[TODO: #1]}}




% In python: print_iterable(['\\bmdefine\\b{0}'.format(x)+'{'+x+'}' for x in 
% string.ascii_letters])

\bmdefine\ba{a}
\bmdefine\bb{b}
\bmdefine\bc{c}
\bmdefine\bd{d}
\bmdefine\be{e}
% \bmdefine\bf{f}  # Clashes with a standard command
\bmdefine\boldf{f}
\bmdefine\bg{g}
\bmdefine\bh{h}
\bmdefine\bi{i}
\bmdefine\bj{j}
\bmdefine\bk{k}
\bmdefine\bl{l}
\bmdefine\bm{m}
\bmdefine\bn{n}
\bmdefine\bo{o}
\bmdefine\bp{p}
\bmdefine\bq{q}
\bmdefine\br{r}
\bmdefine\bs{s}
\bmdefine\bt{t}
\bmdefine\bu{u}
\bmdefine\bv{v}
\bmdefine\bw{w}
\bmdefine\bx{x}
\bmdefine\by{y}
\bmdefine\bz{z}
\bmdefine\bA{A}
\bmdefine\bB{B}
\bmdefine\bC{C}
\bmdefine\bD{D}
\bmdefine\bE{E}
\bmdefine\bF{F}
\bmdefine\bG{G}
\bmdefine\bH{H}
\bmdefine\bI{I}
\bmdefine\bJ{J}
\bmdefine\bK{K}
\bmdefine\bL{L}
\bmdefine\bM{M}
\bmdefine\bN{N}
\bmdefine\bO{O}
\bmdefine\bP{P}
\bmdefine\bQ{Q}
\bmdefine\bR{R}
\bmdefine\bS{S}
\bmdefine\bT{T}
\bmdefine\bU{U}
\bmdefine\bV{V}
\bmdefine\bW{W}
\bmdefine\bX{X}
\bmdefine\bY{Y}
\bmdefine\bZ{Z}


\bmdefine\balpha{\alpha}
\bmdefine\bbeta{\beta}
\bmdefine\bgamma{\gamma}

\bmdefine\bdelta{\delta}
\bmdefine\btheta{\theta}
\bmdefine\blambda{\lambda}
\bmdefine\bphi{\phi}
\bmdefine\bxi{\xi}
\bmdefine\bzeta{\zeta}
\bmdefine\boldeta{\eta}
\bmdefine\bpi{\pi}

\bmdefine\bmu{\mu}
\bmdefine\brho{\rho}
\bmdefine\bomega{\omega}
\bmdefine\bOmega{\Omega}
\bmdefine\bPi{\Pi}

\bmdefine\bvarepsilon{\varepsilon}

\bmdefine\bDelta{\Delta}

\bmdefine\bTheta{\Theta}

\bmdefine\bSigma{\Sigma}
\bmdefine\bPsi{\Psi}
\bmdefine\bLambda{\Lambda}



\bmdefine\bzero{0}
\bmdefine\bone{1}
\bmdefine\binfty{\infty}

 \newcommand{\indicator}{\mathbbm{1}}


% In python 
% print_iterable(['\\newcommand{\\'+'{0}cal'.format(x)+'}{\\mathcal{'+x+'}}' 
% for x in string.ascii_uppercase])
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

